dMath: Distributed Linear Algebra for DL

The paper presents a parallel math library, dMath, that demonstrates leading scaling when using intranode, internode, and hybrid-parallelism for deep learning (DL). dMath provides easy-to-use distributed primitives and a variety of domain-specific algorithms including matrix multiplication, convolutions, and others allowing for rapid development of scalable applications like deep neural networks (DNNs). Persistent data stored in GPU memory and advanced memory management techniques avoid costly transfers between host and device. dMath delivers performance, portability, and productivity to its specific domain of support.

==> system_arch.tex <==
\label{sec:system_architecture}
The \textit{dMath}
 library provides for performance-portable parallel programs, as described in section~\ref{sec:dmath-architecture}.  It is noteworthy that 
the underlying hybrid, heterogeneous COTS parallel architecture that Samsung Electronics has created would be hard for developers to program
directly, in part because of memory and network hierarchies, multiple APIs, and parallel programming models.  With \textit{dMath}, 
the Samsung architecture delivers performance of cost-effective, 
high performance parallel algorithms to end users without requiring extensive explicit parallel programming experience.
%with systems based integration of commodity off the shelf (COTS) technologies.  

As illustrated in Figure~\ref{fig:hw-architecture}, the heterogeneous
architecture utilized consists of x86-64 servers (multicore
Haswell Xeons \cite{IA-Haswell}) connected by EDR
InfiniBand \cite{EDR-IB}.  We utilize the dual PCI-Gen3 buses to
support up to eight NVIDIA GP-GPU's and one InfiniBand EDR network
adapter per scalable server unit root complex.  At present, we utilize
NVIDIA K80 GPU's \cite{NVIDIA-K80}, but this architecture is suitable
for use with next-generation Maxwell \cite{NVIDIA-Maxwell} and Pascal
GP-GPU's \cite{NVIDIA-Pascal} too.

The PCIe 3.0 crossbar switch fills an essential role, becaues it provides 
low-latency switching, and full bandwidth communication between any
GPU pair. For instance, at any given moment, four GPUs can communicate and the host could be
communicating via IB at full PCIv3 speeds. As
long as one maintains pairwise communication between two devices,
communication does not degrade, and there is no congestion.
Many of the subroutines within \textit{dMath} are aware of the importance to use one-to-one communication to maintain optimal use of the hardware.  
If we were to compare this COTS architectures having only
two GPUs per root-complex we can see from
Table~\ref{table:comm_mediums_latency} and \ref{table:comm_mediums_bw}
that the denser root complex scenario that utilizes CUDA P2P, and the
PCIe 3.0 crossbar switch, is favored over shared-memory or Internode
IB EDR for most use cases.

%{\em We need to emphasize the relatively low-end role of the
%Haswell cores... support GPUs, help with message
%passing, support staging of I/O, etc.}

\begin{figure}[!t]
\centering
%\includegraphics[width=\columnwidth]{samsung_architecture}
\includegraphics[width=2.0in]{Figures/ipdps_figure1bb}
\caption{Samsung Heterogeneous Multicomputer Node Architecture.}
\label{fig:hw-architecture}
\end{figure}

%{\em Notes:  Compare storage of DB in SSD, RAID 10 Disk array through IB, Host Memory (NUMA issues)
%Loading of data from a single process is a large bottleneck.
%Ability to have each worker load their own data, allowing for high throughput
%By having loading asynchronous, image loading can be done while other work is going on, taking advantage o\
%f times with low CPU / PCI bus occupancy.
%RAM disk allows for random access when loading the data
%}

